Learning Optimal Control and Dynamical Structure of Global Trajectory Search Problems with Diffusion Models

Spacecraft trajectory design is a global search problem, where previous work has revealed specific solution structures that can be captured with data-driven methods. This paper explores two global search problems in the circular restricted three-body problem: hybrid cost function of minimum fuel/time-of-flight and transfers to energy-dependent invariant manifolds. These problems display a fundamental structure either in the optimal control profile or the use of dynamical structures. We build on our prior generative machine learning framework to apply diffusion models to learn the conditional probability distribution of the search problem and analyze the model's capability to capture these structures.

==> sections/expected_results.tex <==
\section{Expected Results}

Firstly, we will present the groundtruth solution structures of the two global trajectory search problems in the CR3BP by solving them with uniformly sampled initial guesses and various parameter values.
For the hybrid cost function example, we aim to show the optimal control structure in the solutions and how it varies with the parameter $\alpha$ as the weight of the two objectives.
As the objective moves from minimum fuel ($\alpha=1$) to minimum time-of-flight ($\alpha=0$), the locally optimal solutions will transit from bang-bang control profiles for the thrust magnitude to maximal thrust magnitude which supports the theoretical results.
For the energy-dependent invariant manifolds as variable terminal boundary condition example, we aim to show the use of dynamical structures in the groundtruth solutions.
We will present the basin structure on the invariant manifold in the locally optimal solutions and also how these basins on the manifold vary as we change the energy levels $\alpha$ of the corresponding halo orbit.

Secondly, we will leverage a conditional diffusion model with the AmorGS framework to train on the collected locally optimal solutions of these two global trajectory search problems.
We aim to show that our diffusion models can capture those fundamental optimal control structures and the use of dynamical structures from the collected solutions and replicate them in the diffusion samples.
The diffusion model can also use the parameter $\alpha$ as the conditional input and learn how those structures vary with respect to the parameter value of $\alpha$.

Finally, we will use diffusion model samples as the initial guesses for these two global search problems with unseen parameter value $\alpha$ and present the improvement in the computational efficiency.
We will demonstrate that when the diffusion model is able to predict solutions to the new problems with a similar structure as the groundtruth, it will take the solver $\pi$ much less time to converge and thus the global search on the new problems will be accelerated.


